Learning and Trust in Auction Markets

In this paper, we study behavior of bidders in an experimental launch of a new advertising auction platform by Zillow, as Zillow switched from negotiated contracts to using auctions in several geographically isolated markets. A unique feature of this experiment is that the bidders in this market are real estate agents that bid on their own behalf, not using third-party intermediaries. To help bidders, Zillow also provided a recommendation tool that suggested a bid for each bidder. Our main focus in this paper is on the decisions of bidders whether or not to adopt the platform-provided bid recommendation. We observe that a significant proportion of bidders do not use the recommended bid. Using the bid history of the agents we infer their value, and compare the agents' regret with their actual bidding history with results they would have obtained following the recommendation. We find that for half of the agents not following the recommendation, the increased effort of experimenting with alternate bids results in increased regret, i.e., they get decreased net value out of the system. The proportion of agents not following the recommendation slowly declines as markets mature, but it remains large in most markets that we observe. We argue that the main reason for this phenomenon is the lack of trust in the platform-provided tool. Our work provides an empirical insight into possible design choices for auction-based online advertising platforms. While search advertising platforms (such as Google or Bing) allow bidders to submit bids on their own, many display advertising platforms (such as Facebook) optimize bids on bidders' behalf and eliminate the need for bids. Our empirical analysis shows that the latter approach is preferred for markets where bidders are individuals, who don't have access to third party tools, and who may question the fairness of platform-provided suggestions.

==> Sections/abstract-new.tex <==
Auction theory analyses market designs by assuming all players are fully rational.
In this paper we study behavior of bidders in an experimental launch of a new advertising
auction platform by Zillow, as Zillow switched from negotiated contracts to using auctions
in several geographically isolated markets. A unique feature of this experiment is that the
bidders in this market are local real estate agents that bid in the auctions on their own behalf,
not using third-party intermediaries to facilitate the bidding. To help bidders,  Zillow also provided a recommendation tool that suggested the bid for each bidder.

Our main focus in this paper is on the decisions of bidders whether or not to adopt the platform-provided bid recommendation. We observe that a large proportion of bidders does not use the recommended bid. However, for most agents the increased effort of experimenting with alternate bids doesn't result in increased value. We compare the agents regret with their actual bidding history with results they would have obtained consistently using the bidding recommendation. For the agents that change their bids frequently, and only less than 7\% of the agents manage to do better than the recommendations. The proportion of agents not following the recommendation slowly declines as markets mature, but it remains large in most markets that we observe. We argue that the main reason for this phenomenon is the lack of trust that the bidders have in the platform-provided tool.

Our work provides an empirical insight into possible design choices for auction-based online advertising platforms. While search advertising platforms (such as Google or Bing) allow bidders to submit bids on their own and there is an established market of third-party intermediaries that help bidders to bid over time, many display advertising platforms (such as Facebook) optimize bids on bidders' behalf and eliminate the need for the bidders to bid on their own or use intermediaries. Our empirical analysis shows that the latter approach is preferred for markets where bidders are individuals, who don't have access to third party  tools, and who may question the fairness of platform-provided suggestions.


==> Sections/abstract.tex <==
Auction theory analyses market designs by assuming all players are fully rational.
In this paper we study behavior of bidders in an experimental launch of a new advertising
auction platform by Zillow, as Zillow switched from negotiated contracts to using auctions
in several geographically isolated markets. A unique feature of this experiment is that the
bidders in this market are local real estate agents that bid in the auctions on their own behalf,
not using third-party intermediaries to facilitate the bidding. To help bidders,  Zillow also provided a recommendation tool that suggested the bid for each bidder.

Our main focus in this paper is on the decisions of bidders whether or not to adopt the platform-provided bid recommendation. We observe that a large proportion of bidders does not use the recommended bid, resulting
in them achieving worse outcomes. This proportion slowly declines as markets mature, and more bidders use suggested bids, but it remains large in most markets that we observe. We argue that the main reason for this phenomenon is the lack of trust that the bidders have in the platform-provided tool.

Our work provides an empirical insight into possible design choices for auction-based online advertising platforms.
While search advertising platforms (such as Google or Bing) allow bidders to submit bids on their own and there
is an established market of third-party intermediaries that help bidders to bid over time, many display advertising
platforms (such as Facebook) optimize bids on bidders' behalf and eliminate the need for the bidders to bid on
their own or use intermediaries. Our empirical analysis shows that the latter approach is preferred for markets where bidders are individuals, who don't have access to third party  tools, and who may question the fairness of platform-provided suggestions.


==> Sections/data_experiment_description.tex <==
\subsection{Data Description}
Our data come from Zillow ad-auctions in 57 regions until the early August of 2015. On average, in each region there are 10.7 agents who participate in the ad-auctions. The data is presented in time intervals, with a start date and an end date, for which the agents submit their bids. Along with the agents' bids, the data include the agents' monthly budgets for that time interval, the reserve price of the ad-auctions for the region and recommended (suggested) bid of the system to the agent at the start of the period at the time when the agent submitted her bid (the start of the time interval). The estimated monthly impression volume of the ad-auction for the future month (from the start date of each bid) is also available from the data. This estimated impression volume is used by Zillow to suggest a proper bid to the agents. Basic statistics of this data set can be found in table \ref{Tab:AllRegionsBasicInfo}.

\begin{table}[!ht]
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Information & \multicolumn{4}{|c|}{Selected Regions} & \multicolumn{4}{|c|}{All Regions} \\ \hline
Measurement & Mean & STD & 25 Percentile & 75 Percentile & Mean & STD & 25 Percentile & 75 Percentile\\ \hline
Number of agents & 19.33 & 2.29 & 18.0 & 20.75 & 10.74 & 5.32 & 6.0 & 15.0 \\ \hline
Bids & 23.94 & 14.14 & 17.3 & 19.31 & 18.79 & 9.71 & 14.06 & 23.84 \\ \hline
Budgets (daily) & 8.92 & 3.0 & 6.31 & 11.71 & 9.22 & 4.96 & 5.9 & 12.44 \\ \hline
Active duration & 85.97 & 10.38 & 78.03 & 91.5 & 96.04 & 20.74 & 86.53 & 107.33 \\ \hline
Reserve price & 11.65 & 7.03 & 7.99 & 10.74 & 13.39 & 9.55 & 6.0 & 16.93 \\ \hline
Bid changes & 0.73 & 0.26 & 0.54 & 0.85 & 0.22 & 0.28 & 0.03 & 0.32 \\ \hline
\end{tabular}
\caption{Basic information for all regions and the selected regions. Bids, reserve prices and budgets are per 1000 impressions. Active Duration is in days. Bid changes is the average number of agents that change their bid per day in a region. The average of bids, budgets and active duration has been calculated for each agent first and then their averages has been taken over all agents of each region.}
\label{Tab:AllRegionsBasicInfo}
\end{center}
\end{table}


Our second data-set, contains the actual daily impression volumes of each region for a shorter period of time. Since this time period is almost half of the time period when we have the ad-auction data, we use this data-set to adjust the impression volume estimates of the first data-set. This adjustment is done because we observed that the available impression volume has a distinct pattern in all regions, for instance on Sundays and Mondays the impression volume is more than that of other weekdays. Therefore, we are adding the impression volume fluctuations pattern of each region from the actual impression volumes to the region's impression volume estimate for our experiments. This pattern can be seen in figure \ref{Fig:ImpressionFluctuations}.

\begin{figure}[!ht]
\begin{center}
  \includegraphics[width=5.7in]{Figures/WeeklyImpFluctuations.png}
  \caption{Impression volume fluctuations in weekdays shown for 6 regions with the most number bid changes. The weekday's impression volume of each region is normalized by the average daily impression volume of that region.}
  \label{Fig:ImpressionFluctuations}
  \end{center}
\end{figure}

\subsection{Data Processing and Experiments Description}
We are mostly interested in regions for which there is enough data to get meaningful conclusions with regards to agents behavior. In order to do this we first filter the regions where the number of participating agents is 15 or less, which gets down the number of regions from 57 to 12. Another important measure is the number of bid changes per day in these regions, i.e. on average how many agents change their bid per day in a region. This number on average across these 12 regions is 0.43. We filter the regions for which the average number of bid changes across all the agents in that region is less than the average. This gives us a total of 6 regions for which we run most of our experiments. The information about these regions is available in table \ref{Tab:RegionBasicInfo}. The comparison between basic stats of the selected regions and all regions is available in table \ref{Tab:AllRegionsBasicInfo}.

\begin{table}[!ht]
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Region Name & Region 1 & Region 2 & Region 3 & Region 4 & Region 5 & Region 6 \\ \hline
Number of agents (before filtering) & 20 & 23 & 18 & 21 & 16 & 18 \\ \hline
Average bid changes per day & 1.239020 & 0.913344 & 0.65 & 0.548335 & 0.540329 & 0.513930 \\ \hline
Agents in clusters 1,2,3 (after filtering) & 5,5,4 & 5,6,4 & 6,5,1 & 3,2,2 & 8,3,3 & 3,6,1 \\ \hline
\end{tabular}
\caption{Basic information for the 6 selected regions. Filtering removes the agents that are in auction for less than 7 days or do not change their bid at all.}
\label{Tab:RegionBasicInfo}
\end{center}
\end{table}

In each region, an important measurement that indicates activity of each agent is the agent's average number of bid changes per day. Across the selected 6 regions, the histogram of bid change frequencies is shown in figure \ref{Fig:HistBidChangeFrequencies}. We run k-mean clustering algorithm using this measurement to partition the agents inside each region into 3 clusters, agents in cluster 1 and cluster 3 have the lowest and the highest number of bid changes per day respectively. For presenting the results, we remove the agents who are active for less than a week or do not change their bid at all. We also filter the agents whose value cannot be inferred in the results of the no regret learning algorithms in that section. The former and latter is done before and after clustering of the agents, respectively.

\begin{figure}[!ht]
\begin{center}
  \includegraphics[width=5.7in]{Figures/BidUpdateFreqencyHist.png}
  \caption{Histogram of bid change frequencies across the 6 selected regions.}
  \label{Fig:HistBidChangeFrequencies}
  \end{center}
\end{figure}

Another important observation is that agents tend to follow the recommended bid as they stay more in the auction. In order to see this pattern, for each agent, we calculated the fraction of time when she follows the recommended bid in the following months after she joins the system. The average of this number over agents across the 6 selected regions is shown in figure \ref{Fig:FollowingSugBidOverTimeAllReg}. When agents are separated by their clusters, this measurement shows the correlation between frequency of bid changes and following the recommended bid. Figure \ref{Fig:FollowingSugBidOverTimeClusters} shows this measurement for agents in different clusters. This shows agents who are more willing to update their submitted bids, decide to follow the suggested bid sooner and more often than the other agents.

\begin{figure}[!tbp]
\hspace{-1.3cm}
\begin{minipage}[b]{0.5\textwidth}
\begin{center}
  \includegraphics[width=3.5in]{Figures/FollowingSugBidOverTimeAllReg.png}
  \caption{Average fraction of time agents follow the recommended bid across the 6 selected regions.}
  \label{Fig:FollowingSugBidOverTimeAllReg}
  \end{center}
\end{minipage}
\hspace{1.5cm}
\begin{minipage}[b]{0.5\textwidth}
\begin{center}
  \includegraphics[width=3.5in]{Figures/FollowingSugBidOverTimeClusters.png}
  \caption{Average fraction of time agents follow the recommended bid separated by clusters.}
  \label{Fig:FollowingSugBidOverTimeClusters}
  \end{center}
\end{minipage}
\end{figure}

\subsection{Simulating the Ad-auctions}
We calculate the outcome of the ad-auctions separately for each region. For each day, we find the set of agents who have active bids in that day, as well as their bid, their daily budget (which is calculated from the monthly budget and the leftover from the previous days), and the region's reserve price. We use this information to simulate the auction for that day by calculating each agent's filtering probability ($\pi_i$), expected payment and expected share of that day's impression volume. The filtering probabilities are used for budget smoothing described in sections \ref{?} and \ref{?}. It is important to note that none of the agents are removed before finding the outcome of these simulations and these simulations are do not consider the clustering of the agents.

For finding the filtering probabilities, we use the framework described in section \ref{?} and the iterative algorithm of section \ref{?}. One of the main challenges for finding the filtering probabilities is that in each iteration, given the set of previous filtering probabilities, computing the expected cost (eCPM) and expected impressions share (eQ) for all agents can take exponential time in number of agents. Considering the fact that we want to run the simulations for every day and each region separately, these calculations can significantly increase the running time of our simulations. In order to get around this issue, we use the fact that in each underlying GSP, only impressions of the first four agents are eligible to be shown, as well as the fact that the filtering probabilities of agents are independent. Our algorithm runs in polynomial time (in number of agents) and calculates eQ and eCPM given a set of filtering probabilities.

For each agent $i\in[I]$, our algorithm first (lines $[3,6]$) computes the expected impression share of the agent $eQ_i$. Note that $eQ_i$ only depends on the number of unfiltered agents ($r$) that have a higher bid than $i$ and the reward of $i$'s rank ($\gamma_{r+1}$). Since $i$ can only win impressions when she is in one of the first four ranks, the running time of this computation is $O(I^4)$ for each agent. After finding the expected impression share of $i$, we calculate $eCPM_i$ by using $eQ_i$. In order to do this, we use the fact that the filtering probabilities of agents are independent. Furthermore, the expected cost per impression for agent $i$ is only a function of bid of agents who are bidding lower than $i$ and their filtering probabilities. So by calculating the expected cost per impression and multiplying it by the expected impression share of agent $i$, we can calculate her expected cost $eCPM_i$. Recall that for each agent $i$, in order to calculate the total expected number impressions that she wins in the auction and her expected spent, it is enough to multiply $eQ_i$ and $eCPM_i$ by $\pi_i$. Furthermore, the total running time of each iteration of finding the filtering probabilities with this new algorithm is $O(I^5)$ instead of $O(I2^I)$.

The running time of this algorithm can be improved significantly. The most expensive computation in this algorithm is computing $p_{i,r}(\pi)$ for all the agents. For each agent, it takes $O(I^3)$ to find all the configurations where there are $r\in [0,3]$ agents who are not filtered and have higher bid than $i$. For each configuration, it takes $O(n)$ to compute its probability. By using dynamic programming, we can compute $p_{i,r}(\pi)$ by computing the conditional probabilities that agent $i-1$ is getting filtered or not. For each agent $i$, these conditional probabilities can be computed by using the $p_{i-1,r}(\pi)$ probabilities for $r \in [0,3]$ in $O(1)$. This reduces the running time of computing $p_{i,r}$ for all agents from $O(I^5)$ to $O(I)$. Furthermore, the running time of calculating eCPM can be improved for each agent in a similar way: instead of computing eCPM for each agent from scratch, we can compute the price per impression (lines $[7,14]$) from the previous calculations. In order to do this for each agent $i$, it is enough to update this value by removing the impact of agent $i$ from the previous price per impression (which was calculated for agent $i-1$). Note that this calculation will take $O(I)$ for the first agent (with highest bid), but only takes $O(1)$ for all other agents. With these changes, the algorithm will requires $O(1)$ calculations for each agent and it takes linear time ($O(I)$) to calculate eCPM and eQ for all the agents.

\begin{algorithm}[H]
\label{Alg:eCPM}
\DontPrintSemicolon
\KwIn{$b$ (bids), $\pi$ (filtering probabilities), $\gamma$ (auction parameters), $reserve$ (the reserve price)}
\KwOut{$eCPM,eQ$}
Let $\{1,2,\ldots,I\}$ be the list of all agents such that $b_1\geq b_2\geq \ldots \geq b_I$\;
\For{$i \in [I]$}{
Let $eQ_i=0$\;
\For{$r \in [0,3]$}{
Let $p_{i,r}(\pi)$ be the probability that exactly $r$ agents from $[1,i)$ are not filtered.\;
$eQ_i=eQ_i+\gamma_{r+1}.p_{i,r}(\pi)$\;
}
%$eQ_i=\pi_i.eQ_i$\;
Let $j=i+1$\;
Let $eCPM_i=0$\;
\While{$j\in [I]$ and $b_j>reserve$}{
Let $q_{i,j}(\pi)$ be the probability that from all the agents $(i,j]$, only $j$ is not filtered\;
$eCPM_i=eCPM_i + b_j.q_{i,j}(\pi)$\;
$j=j+1$\;
}
Let $q_i(\pi)$ be the probability that all agents from $(i,I]$ are filtered.\;
$eCPM_i=eCPM_i + reserve.q_i(\pi)$\;
$eCPM_i= eQ_i.eCPM_i$
}
\caption{Calculating eCPM and $eQ$ of agents.}
\Return $eCPM,eQ$
\end{algorithm}
